Clique: Spatiotemporal Object Re-identification at the City Scale

Object re-identification (ReID) is a key application of city-scale cameras. While classic ReID tasks are often considered as image retrieval, we treat them as spatiotemporal queries for locations and times in which the target object appeared. Spatiotemporal reID is challenged by the accuracy limitation in computer vision algorithms and the colossal videos from city cameras. We present Clique, a practical ReID engine that builds upon two new techniques: (1) Clique assesses target occurrences by clustering fuzzy object features extracted by ReID algorithms, with each cluster representing the general impression of a distinct object to be matched against the input; (2) to search in videos, Clique samples cameras to maximize the spatiotemporal coverage and incrementally adds cameras for processing on demand. Through evaluation on 25 hours of videos from 25 cameras, Clique reached a high accuracy of 0.87 (recall at 5) across 70 queries and runs at 830x of video realtime in achieving high accuracy.

==> ack.tex <==
% !TeX root = main.tex

%\section*{Acknowledgments}
\begin{acks}
The authors from Purdue were supported in part by NSF Award 1846102, 1718702, and a Google Faculty Award. 
\end{acks}

==> discussion.tex <==
% !TeX root = main.tex

\section{Discussions}
\label{sec:discussion}
%\paragraph{Scalability}
%Indexing and incremental sampling contributes to \sys{} scalability.
%Also depends on data/rarity of objects.

% \paragraph{How is \sys{} related to sota}
%They does not change this problem that reid is expensive;
%sota works has close accuracies around 0.7-0.8; even more expensive with diminishing accuracy growth



==> fig-e2e-overall.tex <==
% !TeX root = main.tex

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.99\textwidth]{figs/eval/e2e/e2e-quali.pdf}
    \caption{Qualitative end-to-end performance comparisons}
\label{fig:e2e-quali}
\end{figure*}

\begin{figure*}[ht]
\centering
    \includegraphics[width=0.99\textwidth]{figs/eval/e2e/e2e-quant.pdf}
    \caption{Quantitative end-to-end performance comparisons}
\label{fig:e2e-quant}
\end{figure*}

==> fig-incremental.tex <==
% !TeX root = main.tex

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/query.pdf}
    \caption{\sys{}'s incremental sampling}
    \label{fig:query}
\end{figure}

==> fig-input.tex <==
% !TeX root = main.tex

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/eval/input/input-camera.pdf}
    \caption{\sys{}'s incremental sampling}
    \label{eval:input}
\end{figure}

==> fig-thresholds.tex <==
% !TeX root = main.tex

\begin{figure}
\centering
\includegraphics[width=.99\linewidth]{figs/eval/thresholds/thresholds.pdf}
\caption{The impact of thresholds}
\label{fig:thresholds}
\end{figure}

==> fig-viewport.tex <==
% !TeX root = main.tex

\begin{figure}
\centering
\includegraphics[width=.99\linewidth]{figs/motiv-viewport.pdf}
\caption{Distribution of object features from the same/different viewport}
\label{fig:viewport}
\end{figure}

==> preprocess.tex <==
% !TeX root = main.tex

\section{Clustering Feature Vectors}
\label{sec:clustering}

\Note{Section title must reflect our key idea}
\notettx{Some key questions on clustering; justify design points should be here}
\notettx{individuals are not good; consecutive frames}
\notettx{clustering is orthogonal to feature extraction; why sift does not work}
\subsection{Rationales}
To enable real-time indexing at video ingestion, \sys{} depends on two of the three prerequisites learned during system setup.

\Note{Need justifying. Why we do this? What's the rationale?}

\paragraph{Benefits of clustering feature vectors}
\Note{This comes in too late. Besides, we need to provide experiments for motivation}

We choose a simple yet effective clustering technique, i.e., k-means clustering~\cite{kmeanspaper} for two reasons.
\begin{myitemize}
\item 
First, unlike object tracking algorithms, clustering is robust on sparse samples.

\item 
Second, k-means clustering performs clustering based-on the characteristics of a group of feature vectors by minimizing within-cluster variances across all clusters. 
It significantly reduces misclassifications for visually similar vehicles that are caused by NN's internal limitations.
\end{myitemize}

\noindent Another well-known clustering algorithm, e.g., hierarchical clustering~\cite{hc}, which hierarchically merges most similar pair of data points or tentative clusters.
However, hierarchical clustering, though straightforward, does not fundamentally remove the internal limitations caused by DNNs on vehicle re-identifications workloads: the merge starting from two individual feature vectors is arbitrary and will easily ends up with cases of multiple vehicles in the same cluster.

\Note{Need justifying clustering. How to train the regression model is well known (1-2 sentences are enough)}

\paragraph{Training K prediction regression model}
To perform effective K-means clustering on the feature vectors, it is crucial to have an accurate K.
% However, the value of K cannot be known beforehand, and therefore we propose to train a simple linear regression model based-on historical data for K-prediction when conducting K-means clustering.
% The estimated K should not deviate from the true K because then the clustering result accuracy will be severely compromised.
We propose to learn the number of vehicles K based-on a simple linear regression model, and \sys{} only needs to collect two variables by running object detection on each time window, i.e., the total number of bounding boxes $x_1$ extracted and the total number of frames $x_2$ that contains vehicles. 
We add three virtual variables that relates to the ratios between the two measures as well: $x_3 = (x1/x2)^2$, $x_4 = (x1/x2)$, and $x_5 = (x2/x1)$, which composes the input $\mathbf{x}$ as $[x_1, x_2, x_3, x_4, x_5]$.
The parameters vector $\mathbf{a}$ and the intercept $b$, as shown in Equation~\ref{regression}, is learned. 
\begin{equation}
\label{regression}
    K = \mathbf{ax}+b
\end{equation}

\noindent\sys{} learns this regression model during system setup and will apply the model to predict K during video ingestion.

==> query.tex <==
% !TeX root = main.tex

\section{Query Execution Planning}
\label{sec:query}

\Note{Section title must reflect our key idea}

\sys{} plans a simple yet concrete incremental query execution based-on cameras votes on \stp s.

\input{fig-incremental}

\Note{Missing justification -- why incremental sampling? In fact, we sample cameras instead of frames. Why is that?}

\subsection{Rationales}
The incremental sampling on cameras saves the appearances of target vehicle undermined by the viewport discrepancy while also saves compute cost by avoiding running NNs on promising \stp s.

\paragraph{Sampling cameras rather than frames}
\sys{}'s sampling majorly explores the redundancy of cameras, which is different from typical prior systems~\cite{videostorm,noscope,focus,vstore,chameleon} that explores on frame temporal redundancy.

% The rationale behind the above workflow of incremental sampling is to minimize the compute costs on pending query workloads upon the ingestion indexes while not losing the accuracy.
For \sys{}, two major factors determine the query execution speed:
% \item \textit{Low/high thresholds} 
% As mentioned in Section~\ref{sec:preprocess}, \sys{}'s incremental sampling strategies are based-on two thresholds: the aggressive choice of $T_{low}$ ensures high precision while the conservative choice of $T_{high}$ ensures high recall.
% For promising \stp s that have been voted \textit{strong accept} by \primary cameras, the precision is guaranteed so that further examinations are skipped.
% For \stp s that have been voted \textit{weak accept} before the query execution, although recall is guaranteed, there exists a significant portion of false positive \stp s, and a further examination is beneficial to distinguish false \stp s that benefits from good viewports and true \stp s undermined by a bad viewports.
% When \sys{} gets down to \stp s that have been voted \textit{weak reject}, the extra gain only come from some extreme rare cases that a trace of target vehicles in a specific $G$ is missed in the \primary cameras picked.

\paragraph{Choosing of primary cameras}
\notettx{capture as many as possible; why one camera per group, why not two cameras and reduced rate}
During system setup, \sys{} also profiles the video footage inside each group and picks the camera that has the most vehicles appeared as \primary cameras, and those cameras are usually locating in the center of the entire camera group.
Although cameras inside the same camera group have high redundancy, vehicles does not always appear in all the cameras within the group.
As a result, a good choice of \primary cameras avoids those cases when the target vehicle to be searched is missed at ingestion time.
For those cases, the indexes built at ingestion failed to catch the target vehicle's feature vectors, and the corresponding \stp will have a bad initial ranking, and thus will not be re-visited until visiting all above \stp s.
This largely downgrades the query efficiency.
We test the sensitivity of the choices on \primary cameras in Section~\ref{eval:sensitivity}.

The design of \primary cameras is cost efficient yet blind.
First, since the target vehicle's orientation and location is not revealed until query time, the \primary camera's viewport that captures the target vehicle might not be the best among all cameras.
Second, although cameras in the same camera groups shows high redundancy that almost all vehicles are shared among the group, there are rare cases that the the target vehicle is missed in the \primary camera while is presented in other cameras.
In this case, \stp s that contains the target vehicles might be voted as ~\textit{weak reject} before query execution, and is re-visited in comparatively lower priorities.

\paragraph{Indexing on more cameras?}
The alternative designs with more than one \primary cameras is a diminishing return: with a few $\times$ compute costs paid at video ingestion, the query cost paid at query time for average precision to converge does not differ significantly.
We evaluate above alternative designs in Section~\ref{eval:tradeoffs}.

\paragraph{Summary \& implications of incremental sampling}
The design of incremental sampling is crucial to \sys{}'s cost efficiency.
\sys{} exploits sampling on two dimensions, i.e., spatially and temporally.
First, as one of our major key designs, spatial sampling performs sampling on cameras.
Referring to the indexes built during video ingestion, \sys{} incrementally expands to other cameras on demand.
Second, we follow the well-known frame sampling technique adopted by prior work~\cite{videostorm,noscope,focus,vstore,chameleon} to reduce cost based-on frame redundancies.
However, based-on our observations, clustering are robust on low frame rates and clustering accuracy actually does not differ significantly across more than 10$\times$ frame rate differences, so for \sys{}, we do not tune the knob of sampling rates.
\Note{It seems we should state that we focus on camera sampling. Spatial/temporal sampling is old. But favor camera sampling over frame/pixel sampling could be new.}

% \subsection{Real-time sparse indexing}
\subsection{Incremental Query Execution}

\Note{Section title must reflect our key idea}

\Note{What's the top point of this paragraph? It also needs motivation/justification.}

During video ingestion, \sys{} builds sparse yet concrete indexes on a small portion of cameras, i.e., \primary cameras, and the indexes will guide the incremental query execution that will save considerable amount of compute costs.
As the videos continuously ingests into each camera, \sys{} extracts vehicle objects by generic object detectors, e.g., YOLO~\cite{yolo}, and extract the feature vectors by re-identification NN for each vehicle object detected.
Within each time window $TW$ and each camera group $G$, \sys{} runs K-means clustering on all the feature vectors in each $G$ with the $K$ predicted by the regression model learned during system setup.
As a result, the centroid feature vectors from each K clusters $C_1 ... C_K$ are recorded for later query executions.

At query time, the user provides \sys{} with the input feature vector $f_{target}$ extracted by re-id NN from the target vehicle.
For each \stp, \sys{} calculates the feature vector distances $d$s between $f_{target}$ and each of the $K$ centroid feature vectors $C_1 ... C_K$ by L2-norm.
Based-on $d_{min}$ from each \stp, \sys{} derives an initial ranking of all \stp s.
For each \stp, the initial vote is 0, and the weight for each decision is different.
For \textit{strong accept}, the \primary camera adds 2 to the votes; for \textit{weak accept}, the \primary camera adds 1 to the votes; for \textit{weak reject}, the \primary camera adds -1 to the vote.

\noindent For \stp s voted with different tentative decisions, \sys{} adopts different incremental sampling strategies, as shown in Figure~\ref{fig:query}.
\encircle{1} Beginning at the top of the list, if \stp is tagged as \textit{strong accept}, \sys{} accepts these \stp s and skips incremental processing.
\encircle{2} For \stp s tagged as \textit{weak accept}, \sys{} further investigates the vehicle similarity by invoking \pu on the same $TW$ from another camera in the camera group.
If the new camera voted \textit{strong accept} or \textit{weak accept} for this \stp, \sys{} moves \stp onto the output list.
Otherwise, the vote for this \stp drops from 1 to 0 after voted \textit{weak reject}.
\encircle{3} For all \stp s that have a vote $\leq 0$, from the top of those \stp s, \sys{} incrementally runs \pu in the same $TW$ on another camera in the same $G$ and updates each \stp's vote and $d_{min}$ based-on the new results.
The ranking is continuously updated based-on the $d_{min}$ from each \stp.
\sys{} conducts multiple rounds of incrementally sampling on all \stp s that currently has a vote $\leq 0$ from the prior round.
In the end, \sys{} ceases the query execution until that for each \stp, the number of cameras not visited in $G$ cannot turn the negative vote to positive, i.e., even if all the rest of the cameras votes \textit{strong accept}, the final vote is still $\leq 0$.


==> tab-corr.tex <==
% !TeX root = main.tex

\begin{table}[]
% \scriptsize
\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} 
\hline 
& $C1$ & $C2$ & $C3$ & $C4$ & $C5$ & $C6$ & $C7$  \\ \hline
Appeared in $\geq 50\%$ cams in $C_i$ & 100\% & 100\% & 64.3\% & 100\% & 95.7\% & 58.5\% & 75\% \\ 
%\hline
% Sharing $\geq50\%$ time (within) &  &  &  &  &  &  & \\ 
\hline
Appeared in $\geq 50\%$ groups & 14.3\% & 12.5\% & 7.1\% & 14.3\% & 4.3\% & 2.4\% & 4.1\%\\ 
%\hline
% Sharing $\geq 50\%$ time (all) & & & & & & & \\ 
\hline

\end{tabular}
\caption{The correlation between cameras groups ($C_1$ to $C_7$) from CityFlow~\cite{cityflow} \textbf{XXX move to eval}}
\label{tab:corr}
\end{table}

\begin{comment}
\begin{table}[]
% \scriptsize
\footnotesize
\centering
\begin{tabular}{|c|c|c|} \hline 
 & VIDs in >50\% cams & VIDs overlaps in >50\% time ranges \\ \hline
C1 & & \\ \hline
C2 & & \\ \hline
C3 & & \\ \hline
C4 & & \\ \hline
C5 & & \\ \hline
C6 & & \\ \hline
C7 & & \\ \hline

\end{tabular}
\caption{The profiled correlation cameras clusters ($C_1$ to $C_7$) from CityFlow dataset}
\label{tab:commonids}
\end{table}
\end{comment}

